Particle production as a function of the underlying event in pp collisions simulated with PYTHIA 8

In this work we present the production of charged particles associated with high-$p_{\rm T}$ trigger particles ($8<p_{\rm T}^{\rm trig.}<15$ GeV /$c$) at mid-pseudorapidity in proton-proton collisions at $\sqrt{s}=5.02$\,TeV simulated with the \textsc{PYTHIA 8} Monte Carlo model. The study is performed as a function of the relative transverse activity classifier, $R_{\rm T}$, which is the relative charged-particle multiplicity in the transverse region ($\pi/3 <|\Delta\phi| <2\pi/3$) of the di-hadron correlations, and it is sensitive to the Multi-Parton Interactions. The evolution of the yield of associated particles on both the toward and the away regions with $3\leq p_{\rm T}^{\rm assoc.}<8$ GeV/$c$ as a function of $R_{\rm T}$ is investigated. We propose a strategy which allows for the modelling and subtraction of the Underlying Event (UE) contribution from the toward and the away regions in challenging environments like those characterised by large $R_{\rm T}$. We found that the signal in the away region becomes broader with increasing $R_{\rm T}$. Contrarily, the yield increases with $R_{\rm T}$ in the toward region. This effect is reminiscent of that seen in heavy-ion collisions, where an enhancement of the yield in the toward region for $0-5\%$ central Pb--Pb collisions at $\sqrt{s}_{\rm NN}=2.76$\,TeV was reported. To further understand the role of the UE and additional jet activity, the transverse region is divided into two one-sided sectors, "trans-max" and "trans-min" selected in each event according to which region has larger or smaller charged particle multiplicity. Based on this selection criterion, the observables are studied as a function of $R_{\rm T}^{\rm max}$ and $R_{\rm T}^{\rm min}$, respectively. The presented results have been published in J. Phys. G 48, no.1, 015007 (2020) and Phys. Rev. D 104, no.1, 016017 (2021).

==> c <==
#!/bin/bash

if [ -z "$1" ];then
echo -en "\n\n\tUsage: $0 /path/to/TeX/file\n\n"
echo -en "\tExample: ./c ./alicepreprint_CDS.tex\n\n"
exit 99;
fi

filename=$(basename $1)
extension=${filename##*.}
filename=${filename%.*}

PWD=`pwd`
LOG="${PWD}/compile.log"

rm -vf *.{aux,dvi,log,spl,ps,bbl,blg}

clear;
echo -en "\n\n\tCompiling LaTeX document $1 at `date +"%r"`...\n" &&
pdflatex -shell-escape $1 > /dev/null && 
echo -en "\n\t\tx 1 times ...\t\t\t\t[ OK ]\n" &&

# # bibtex $filename &&

pdflatex -shell-escape $1 > /dev/null && 
echo -en "\t\tx 2 times ...\t\t\t\t[ OK ]\n" &&

pdflatex -shell-escape $1 > /dev/null && 
echo -en "\t\tx 3 times ...\t\t\t\t[ OK ]\n\n" &&
echo -en "Opening $filename.pdf ...\t\t\t\t[ OK ]\n" &&

acroread $filename.pdf 2>/dev/null&
# # # # evince $filename.pdf 2>/dev/null&

